Fed-Sim: Federated Simulation for Medical Imaging

Labelling data is expensive and time consuming especially for domains such as medical imaging that contain volumetric imaging data and require expert knowledge. Exploiting a larger pool of labeled data available across multiple centers, such as in federated learning, has also seen limited success since current deep learning approaches do not generalize well to images acquired with scanners from different manufacturers. We aim to address these problems in a common, learning-based image simulation framework which we refer to as Federated Simulation. We introduce a physics-driven generative approach that consists of two learnable neural modules: 1) a module that synthesizes 3D cardiac shapes along with their materials, and 2) a CT simulator that renders these into realistic 3D CT Volumes, with annotations. Since the model of geometry and material is disentangled from the imaging sensor, it can effectively be trained across multiple medical centers. We show that our data synthesis framework improves the downstream segmentation performance on several datasets. Project Page: https://nv-tlabs.github.io/fed-sim/ .

==> method.tex <==
\section{Methodology}
\label{sec:method}

We aim to learn a generative model $S_\theta$ to synthesize CT volumes and their corresponding labels (in our case voxel segmentation labels). Here, $\theta$ are learnable parameters of our model that we wish to learn from a given CT dataset $D$ with few annotated and several unlabeled volumes. We wish to learn $S_\theta$ such that it captures the \emph{essence} of the dataset $D$, and can generate new samples from its distribution. For our purpose, we split $D$ into training, validation and test sets, where the validation and test sets are labelled. From the training set, we assume a (small) subset is labelled, which we use to train our method. 

%Given a CT dataset $D$ with few annotated volumes, we aim to learn a parametric data simulator (generative model) $S_\theta$, with parameters $\theta$ such that new CT volumes with labels can be sampled from it. We wish to learn the model such that it captures the \emph{essence} of the dataset $D$, and can generate new samples from its distribution. We split $D$ into training, validation and test sets, where the validation and test sets are labelled. From the training set, we assume a (small) subset is labelled, which we use to train our method. 

Our generative model (Fig.~\ref{fig:model}) consists of generating a shape parameter that controls a statistical shape model (SSM) of an organ (heart, in our case) to produce a 3D mesh, and a coarse material map indicating material properties of each voxel in the organ, which when passed through a physics-based CT simulator, gives us a synthetic CT volume with labels. Additionally, we pass single slices of the generated volume (and the label) through a Generative Adversarial Network (GAN)~\cite{park2019semantic}) to enhance and generate final CT slice images.

% \SF{generative process vs parametric simulator not clear}
%\SF{do we need this? it's not clear... what is multi-label masks, etc? we need a clear overview} Our method works by learning to generate parameters for a CT renderer, where the parameters govern the 3D shape of an organ (a heart parametrized by a statistical shape model (SSM) in our case) and tissue-specific material properties (X-ray attenuation coefficient, density) in the volume around the organ. As these simulated CTs utilise multi-label masks/material maps generated from instances of the multi-region SSM, the `ground truth' labels for the regions of interest (to be segmented) are readily available for each image volume. 
 
In Sec.~\ref{ss:shape}, we describe our parametrization of shape and material. Sec~\ref{ss:sim} explains the physics-based CT simulator that takes shape and material as input to produce a CT volume. We introduce our generative model in Sec.~\ref{ss:gen} and explain how we learn it in  Sec.~\ref{ss:learning}. Finally, in Sec.~\ref{ss:federated} we propose how to implement the algorithm in a federated setting across multiple data sites. 

%\subsection{Parametric CT Simulator}
\subsection{Parametric 3D Representation of an Organ}
\label{ss:shape}
We represent an organ using a parametric \emph{shape representation} to generate whole heart meshes, and material properties (X-ray attenuation coefficient, density).
%Given input shape model parameters, and material properties (X-ray attenuation coefficient, density), the simulator uses a \emph{CT renderer} to render the mesh and material properties into a CT volume.

\textbf{Shape Representation:} We opt for a statistical shape model (SSM) based representation to constrain generated shapes to be physically plausible and provide control over the shape using a reduced set of parameters, ensuring tractable learning. In our case, the SSM is a parametric representation of the whole heart and its associated great vessel trunks (pulmonary artery and aorta), including seven regions, namely, the blood pool and myocardium of the left ventricle, the right ventricle, the left and right atria, and the vessels. We estimated our SSM using PCA, following group-wise registration of 20 shapes using the method proposed in~\cite{ravikumar17}. The training shapes used to estimate the SSM were generated from segmentations of cardiac cine-MRIs, provided as part of the multi-modality whole-heart segmentation (MM-WHS) challenge~\cite{zhuang16}.

\textbf{Material Representation:}
 
 \subsection{CT Simulator}
\label{ss:sim}

\textbf{CT Renderer:} We use PYRO-NN \cite{syben2019pyro} as our CT renderer, a python-based CT reconstruction framework which provides cone-beam forward and back-projection operations embedded as Tensorflow layers, enabling easy integration of the renderer within our simulation network. As outlined in \cite{syben2019pyro} projection domain images can be computed as,
\begin{equation}
    \label{eq.fproj}
    \mathbf{A}\mathbf{T} = \mathbf{I}
\end{equation}
\SF{We need to link to notation in 3.1} where, $\mathbf{A}$ is the projection matrix for a given imaging geometry (cone-beam), $\mathbf{T}$ is the object (cardiac shape and associated material map) and $\mathbf{I}$ are its projections. The total X-ray attenuation in the projection images is computed by ray-casting according to the Beer-Lambert law, as described in \cite{maier2013conrad,unberath19} based on the X-ray spectral density and the estimated material map. The material map is a combined representation of the voxel-wise tissue- and energy-dependent linear attenuation coefficient and material density at each point in the object. The generated projection images can be used to reconstruct a 3D CT volume using the filtered back-projection (FBP) algorithm, by computing the pseudo-inverse of the projection matrix. This allows the reconstruction operation to be expressed as,
\begin{equation}
    \label{eq.fproj}
    \mathbf{T} = \mathbf{A}^{T} \mathbf{F}^{H} \mathbf{K F I}
\end{equation}
where, $\mathbf{A}^{T}$ and $\mathbf{F}^{H}$ represent the adjoint operators of the projection matrix and Fourier transform respectively, and $\mathbf{K}$ represents a diagonal filter matrix in the Fourier domain used to compute the pseudo-inverse. As highlighted in \cite{syben2019pyro, wurfl2018deep} these forward and back-projection operators $(\mathbf{A}, \mathbf{A}^{T})$ are differentiable and are implemented as layers in PYRO-NN through which gradients can be efficiently propagated for end-to-end training of CT reconstruction networks. 

\DL{We should cite 7T. W¨urfl, F. C. Ghesu, V. Christlein, and A. Maier,
Deep learning computed tomography, in International Conference on Medical Image Computing
and Computer-Assisted Intervention, pages 432–440,
Springer, 2016. to show these operators are differentiable}
\AK{talk about voxelization here. sizes are mentioned in the generative process}

\subsection{Generative Model}
\label{ss:gen}
Here, we describe our generative model (Fig.~\ref{fig:model}), which first generates shape parameters and a material map, that are passed through the CT simulator to generate a synthetic CT volume with labels. Additionally, we \emph{enhance} the generated CT volume using a conditional Generative Adversarial Network (GAN)~\cite{park2019semantic}.
%Our generative process consists of generating a shape parameter and a coarse material map, which when passed through the CT simulator, gives us a synthetic CT volume with labels. Additionally, we pass single slices of the generated volume (and the label) through a Generative Adversarial Network (GAN)~\cite{park2019semantic}) to enhance and generate final CT slice images. Fig.~\ref{fig:model} depicts this process.

\textbf{Shape/Material Generation:} From a latent vector $z \in \mathcal{Z}$, we generate a shape parameter $\tau_S = G_{\theta_S}(z) \in \mathcal{R}^X$ through Y \AK{details to be filled here} fully connected neural network layers. We also pass $z$ through T layers, to generate a coarse material voxel map $\tau_M = G_{\theta_M}(z) \in \mathcal{R}^{16\times16\times16}$.

\textbf{CT Simulation:} The generated shape parameters $\tau_S$ and material map $\tau_M$ are passed through the CT simulator introduced above to generate a voxelized label map $Y_z \in \mathcal{R}^{128\times128\times128}$ and a CT voxel volume $\tilde{X_z} \in \mathcal{R}^{128\times128\times128}$. Note that the generated CT volume is coarse due to the coarseness of the material map.

\textbf{CT Volume Enhancement:} CT-Images are dependent on factors such as the scanning machine and acquisition protocol at a site, which are not all modelled in our simulator. Additionally, our generated CT volume is a coarse representation. Therefore, we use a GAN to both enhance and translate our simulated CT images to look similar to target images, bridging the gap between simulation and the target dataset. The generated coarse CT volume $\tilde{X}_z$ and label map $Y_z$ are used to generate final high resolution synthetic CT images. Specifically, we utilize GauGAN~\cite{park2019semantic} $(G_{\text{GAN}})$ to take a slice $k$ of $\tilde{X}_{z}$, $Y_z$ and slice index $k$ as input and generate a final CT slice image $X_{z,k}$, with label $Y_{z,k}$ for all slices. We choose GauGAN since is designed to respect semantic shape input, which is the label map in our case. Particularly, 1) we take the $k^{\text{th}}$ slice of $\tilde{X}_z$ and $Y_z$ and 2) create a $128\times128$ slice with a constant value of $\frac{k}{128}$ and concatenate them together as the input to $G_{\text{GAN}}$.

Overall, the generative model can be written succinctly as,
\begin{align*}
    S_z &= \text{SSM}(G_{\theta_S}(z))\\
    \tilde{X}_z, Y_z &= \text{CT}_{\text{sim}}(S_z, G_{\theta_M}(z))\\
    X_{z,k} &= G_{\text{GAN}}(\tilde{X}_{z,k}, Y_{z,k}, k) \quad \forall \: k
\end{align*}
where $S_z$ represents the shape obtained from the SSM with parameters $G_{\theta_S}(z)$.

\subsection{Learning}
\label{ss:learning}
We train our generative model using the Generative Latent Optimization(GLO)~\cite{bojanowski2017optimizing} framework in two stages: pre-training and unsupervised training. First, we pre-train the model using the part of the training set with labels, and then fine-tune the model semi-supervised additionally using the rest of the unlabelled training data. We first introduce the GLO framework and then describe our training stages.

\textbf{GLO~\cite{bojanowski2017optimizing}:} Generative Latent Optimization is a technique for learning generative networks using only reconstruction losses. Particularly, every volume in the training set is coupled with a particular latent vector $z^i$ (initialized from a unit normal distribution), which is simultaneously learnt along with a generation process that transforms $z^i$ into a volume. Learning is done by optimizing reconstruction losses between the generated volume and the corresponding ground truth volume. The set of learnt latent vectors $\{z^i\}$ can be fit to a parametric distribution (\emph{eg.} multivariate normal), which is sampled from to generate new volumes. 

\textbf{Pre-training:} We use the training CT volumes which have ground truth annotations to pre-train the parameter generation module ($G_{\theta_S}$ and $G_{\theta_M}$). Specifically, a shape parameter $\tau_S^i$ and a material map $\tau_M^i$ are generated from a latent vector $z^i \in \mathcal{R}^{d}$ (which is associated with a training CT-image $X^i$ and ground truth segmentation $Y^i$). These parameters are used to synthesize a binary label $Y_z^i$ and a coarse CT volume $\tilde{X}_z^i$ through the CT simulator, which we supervise. We use the mean Intersection-Over-Union (mIoU) metric to learn $G_{\theta_S}$, and a combination of mean-square-error and perceptual loss~\cite{johnson2016perceptual} using all VGG-19~\cite{simonyan2014very} layer features for $G_{\theta_M}$.
\begin{align*}
    L_{\text{IoU}}(\theta_S) &= 1 - \frac{Y_z^i \odot Y^i}{Y_z^i + Y^i - Y_z^i \odot Y^i}\\
    L(\theta_M) &= \norm{\tilde{X}_z^i - \tilde{X}^i}_2^2 + L_{\text{perc}}(\tilde{X}_z^i, \tilde{X}^i)
\end{align*}

where $\tilde{X}^i \in \mathcal{R}^{128\times128\times128}$ is the real CT volume $X^i$ which is trilinearly downsampled to $16\times16\times16$ and upsampled again to simulate coarseness, $\odot$ represents the hadamard product and other operations are element-wise for matrices. $L_\text{perc}$ is implemented following~\cite{park2019semantic}.  Backpropagation through the SSM is done by calculating the gradients using finite-differences on the low-dimensional SSM parameters. \AK{Make it clearer before that the Ys are binary}.

After pre-training $G_{\theta_S}$ and $G_{\theta_M}$, we pre-train our conditional GAN $G_{\text{GAN}}$. Specifically, in this phase, we use a slice $k$ of the ground truth labels $Y^i$ instead of the generated labels $Y_z^i$, and the generated material $\tilde{X}_z^i$ as input to the GAN, and supervise it with the associated real CT Volume $X^i$, using the same loss functions as~\cite{park2019semantic}. Using the ground truth label ensures that the input label and the output image have the same exact shape, resulting in the GAN learning to generate high-resolution CT that respects the input shape.

\textbf{Semi-Supervised Learning:} We utilize the (usually easily available) unlabelled data in the training set to improve our simulation. The abundance of unlabelled data and the cost of annotation makes this a compelling proposition. In this stage, we alternate between training on supervised data (explained above), and training on unsupervised data (the training schedule is discussed in Sec.~\ref{sec:method}). First, we fit a multivariate normal distribution to the latent vectors optimized in the pre-training phase, and sample new random latent vectors $z^i$ for the unlabelled data-points from this distribution. To train unsupervised, we run our full generative process from every $z^i$ to generate a high resolution CT image $X_{z,k}^i$ for some random slice index $k$ from $z^i$ and use the same loss function for the GAN as above to train. This phase allows our model to adapt the model to be able to learn shape and material parameters for data points without ground-truth segmentation annotations. In this phase, we do not update the GAN Discriminator, and observe that it strongly improves training stability.

\subsection{Federated Simulation}
\label{ss:federated}
Medical data (CT Imagery, in our case) is usually available at multiple sites, each with their specific acquisiton parameters and privacy concerns, which makes both consolidating data and training on consolidated data (domain adaptation) difficult\AK{Citation here in medical context?}. With our learnt simulation framework, we demonstrate \emph{federated simulation}, where we learn our simulation models with data from multiple hospitals in a federated fashion. Because of our disentanglement of shape and material from the CT process, we are in an advantageous position where we can learn shape and material parameters across multiple sites, and \emph{render} generated shapes and materials from this global distribution into CT volumes from a particular hospital's distribution through the CT simulator and the site-specific(local) enhancement GAN. This mitigates both issues of data consolidation and domain adaptation.

Fig.~\ref{fig:federated} depicts this process. We learn one $G_{\theta_S}$ and $G_{\theta_M}$ to model the distribution of shapes and materials across sites, and learn a site-specific $G_\text{GAN}$. In every case, we take one step update from each site, accumulate gradients and run a step of gradient descent at the server, and broadcast the updated weights back to the sites. We note that this is a simple federated setting and serves to demonstrate our method; but a real deployment would require additional engineering considerations. Additional details are provided in the supp. material.

% \subsection{Background}

% \subsubsection{Forward Projection}
% Beer-Lambert's law, for monochromatic source spectrum.
% \begin{equation}
%     I(E) = I_{o}(E) \exp\bigg(-\int_{0}^{s}\mu(E,t)dt\bigg)
% \end{equation}
% For polychromatic source,
% \begin{equation}
%     I = \int I_{o}(E)\exp\bigg(-\int_{0}^{s}\mu(E,t)dt\bigg)dE
% \end{equation}
% if we further assume the materials are homogeneous, we can simplify the equation as in \cite{unberath2018deepdrr},
% \begin{equation}
%     I = \int I_{o}(E)\exp\bigg(-\sum_{m \in M} \mu_{m}(E) \int \delta(m,M(t)) \rho(t)dt\bigg)dE
% \end{equation}
% Where $\delta(\cdot,\cdot)$ is the Kronecker delta, $\mu_{m}(E)$ is the material and energy dependent linear attenuation coefficient, and $\rho(t)$ is the material density at position t. Usually CT detector measure signals in the form of logarithmic ration of the initial energy intensity $I_{o}(E)$ and the final energy intensity $I$ as
% \begin{equation}
%     \lambda = \ln\bigg(\frac{I_{o}}{I}\bigg)
% \end{equation}

% To obtain comparable attenuation values for different CT scanners, the value of $\mu$ is converted into Hounsfield units H:
% \begin{equation}
%     H = \bigg(\frac{\mu}{\mu_{H_2O}}-1\bigg)*1000
% \end{equation}

% \subsubsection{Reconstruction}
% The widely known FDK \cite{feldkamp1984practical} also known as filter backprojection(FBP) algorithm. FDK is an approximate reconstruction algorithm for circular cone-beam tomography. Although the algorithm is an approximation, the error rate are usually acceptable. We are using FDK as our reconstruction algorithm and the dual for the gradient of forward projection. The actual reconstruction equation depends on geometry, for simplicity, we assume a 2D circular trajectory and parallel projection. position $x, y$ can be parameterized as
% \begin{equation}
%     x(s) = l\cos{\theta} - s\sin{\theta}
% \end{equation}
% \begin{equation}
%     y(s) = l\sin{\theta} + s\cos{\theta}
% \end{equation}
% \begin{equation}
%     g(l,\theta) = -\ln\frac{I}{I_o} = \int_{-\infty}^{\infty}\int_{-\infty}^{\infty}f(x,y)\delta(x\cos{\theta}+y\sin{\theta}-l)dxdy
% \end{equation}
% Filtered Backprojection:
% \begin{equation}
%     f(x,y)= \int_{0}^{\pi}\bigg[\int_{-\infty}^{\infty}|\rho|G(\rho,\theta)\exp^{-j2\pi\rho l}d\rho\bigg]_{l=x\cos{\theta}+y\sin{\theta}}d\theta
% \end{equation}
% Convolution Backprojection:
% \begin{equation}
%     f(x,y) = \int_{0}^{\pi}\bigg[c(l)*g(l,\theta)\bigg]_{l=x\cos{\theta}+y\sin{\theta}}d\theta
% \end{equation}
%  where $c(l)=F^{-1}\{|\rho|\}$

% \subsubsection{CT Rendering Equation}
% \begin{equation}
%     \mathbf{Ax = p},
% \end{equation}
% Where $\mathbf{A}$ is the projection matrix describing the geometry of the projection, $\mathbf{x}$ is the object under projection and $\mathbf{p}$ is the projection results also called sinogram in medical imaging.
% \begin{equation}
%       \mathbf{x = A^{-1}p} ,
% \end{equation}
% where $\mathbf{A^{-1}}$ is the inverse system matrix and usually are tall matrix thus cannot be inverted directly. The reconstruction can be conducted using the Moore-Penrose Pseudo Inverse
% \begin{equation}
%       \mathbf{x = A^{T}(AA^{T})^{-1}p} ,
% \end{equation}
% Where $A^{T}$ can be implemented as back projection.
% \begin{equation}
%       \mathbf{\widetilde{x} = A^{T}F^{H}KFp} ,
% \end{equation}
% Where $F$ is Fourier transform and $F^H$ is the inverse Fourier transform. K is an diagonal matrix in Fourier Domain. $\widetilde{x}$ is the reconstructed object.

% \subsection{Active Shape Models}
% Our Active Shape Models (ASM) is obtained using principal component analysis (PCA) on a small set of cardiac CT shapes $S$. The shape class mean and covariance can be written as:
% \begin{equation}
%     \tilde{s} = \frac{1}{M}\sum_{i=1}^{M}s_i
% \end{equation}
% \begin{equation}
%     C = \frac{1}{M-1}\sum_{i=1}^{M}(s_i-\tilde{s})(s_i-\tilde{s})^T
% \end{equation}
% The PCA of the shape produces l eigenvectors $\Phi=[\varphi_{1}\varphi_{2}...\varphi_{l}]$ and the corresponding eigenvalues $\mathbf{\Lambda}=diag(\lambda_{1},\lambda_{2},...,\lambda_{l}])$. Then the new shape can be approximated from the following linear generative model:
% \begin{equation}
%     s \approx \tilde{s} + \Phi b
% \end{equation}
% where $b$ are shape parameters.

% \subsection{Learnable Parameters}
% We have learnable shape deformation parameters which include shape parameters $b$ for the top 14 eigenvectors and rigid transformation parameters (see Table ~\ref{tab1}). We also have learnable device related parameters such as \textit{Source to Detector Distance (SDD)}, \textit{Source to Isocenter Distance (SID)}, \textit{detector shape}, \textit{detector spacing}, \textit{projection angular range}, \textit{number of projection}, \textit{source spectrum energy}, \textit{photon density} (see Table ~\ref{tab2}).

% \begin{table}[h!]
% \centering
% \caption{Shape Parameters.}\label{tab1}
% \begin{tabular}{ |l|l| } 
%  \hline
%  Name & Range \\
%  \hline
%  PCA weights & -1.5-1.5 \\ 
%  \hline
%  scale & 0.5-2.0 \\
%  \hline
%  rot\_x & -30-30 \\ 
%  \hline
%  rot\_y & -30-30 \\ 
%  \hline
%  rot\_z & -30-30 \\ 
%  \hline
%  tran\_x & -0.3-0.3 \\ 
%  \hline
%  tran\_y & -0.3-0.3 \\ 
%  \hline
%  tran\_z & -0.3-0.3 \\ 
%  \hline
% \end{tabular}
% \end{table}

% \begin{table}[h!]
% \centering
% \caption{Device Parameters.}\label{tab2}
% \begin{tabular}{ |l|l| } 
%  \hline
%  Name & Range \\
%  \hline
%  SDD & 800mm-1600mm \\ 
%  \hline
%  SID & 200mm-700mm \\
%  \hline
%  detector\_shape & 128mm-384mm \\ 
%  \hline
%  detector\_spacing & 1.0mm-2.0mm \\ 
%  \hline
%  angular\_range & $\pi$-$2\pi$ \\ 
%  \hline
%  num\_projection & 180-360 \\ 
%  \hline
%  spectrum\_energy\_cov & 0.5-2.0 \\ 
%  \hline
%  photon\_density\_cov & 0.5-2.0 \\ 
%  \hline
% \end{tabular}
% \end{table}

% \subsection{Stage I: Shape and Material model jointly training}
% We use GLO\cite{bojanowski2017optimizing}, which is a recently proposed latent regression generative model, to train a join generative model of the shape and material model. As in \cite{bojanowski2017optimizing}, we first initialize a set of d-dimentional random vectors ${z_1,...,z_N}$ sampled from a normal distribution, where $z_i \in Z$. Then we pair the dataset of images in our case, it is the segmentation volume of patients, the low resolution material map obtained by applying trilinear interpolation of the original image, with the random vectors, obtaining the dataset $\{(z_1,s_1,m_1),...,(z_N,s_1,m_N)\}$. The generative model of the shape $G_{\theta_S}: Z \rightarrow S$ is parameterized by an Neural Network that maps $zi \in Z$ to the shape space $S \in R^{21}$. Similarly, the generative model of the material $G_{\theta_M}: Z \rightarrow M$ is also parameterized by an Neural Network that maps $zi \in Z$ to the material space $M \in R^{16x16x16}$.\\
% The generated shape parameters are then passed to an non-differentiable layer which applies learned PCA weights and rigid transformation to an mean mesh and then the transformed mesh is voxelized into a voxel. We obtain the gradient using numerical method. Since the output voxel is a volume mask where 1 indicates foreground and 0 indicates background, we do not need to threshold the predication map like other methods where their final output is a probability map. Due to this, we can use mean Intersection over Union (mIoU) as our loss directly. 
% \begin{equation}
%     L_{mIoU} = 1.0 - \frac{1}{N}\sum_{i=1}^{N}\bigg[\frac{TP}{TP+FP+FN}\bigg]
% \end{equation}
% The generated material $M$ is represented as an low-resolution attenuation coefficient for the CT volume. We then pass $M$ into the CT simulator with predefined machine related parameters $D$ which we assume each hospital can modify it based on its machine configuration to obtain $\widetilde{M} = T(M, S, D)$ which is an nosier version of $M$ after applying device related artifacts. We trained the material model using a combination of MSE loss and VGG loss, also known as perceptual loss.
% \begin{equation}
%     L_{material} = MSE(\widetilde{M}, M_{real}) + VGG(\widetilde{M}, M_{real})
% \end{equation}\\
% Finally we jointly learn the parameters $\theta_S$ of the shape generator, $\theta_M$ of the material generaor and
% \begin{equation}
%     min_{\theta_{S}, \theta_{M}} \frac{1}{N}\sum_{i=1}^{N}\bigg[min_{z_i}\big[L_{mIOU}(G_{\theta_S}(z_i), s_i) + L_{material}(G_{\theta_M}(z_i), m_i)\big] \bigg]
% \end{equation}

% \subsection{Stage II: Local Enhancer training}
% After Stage I, we can generate new shape, material pairs $(s_i, m_i)$ by sampling random $z_i$ from an fitted Gaussian distribution. Since the material $m_i$ generated in Stage I is still in a very course level, we want to train an local enhancer to enhance fine details. We treat it as an image-to-image translation task that translate a low-resolution CT image into a high-resolution CT image with additional conditions on segmentation mask. We trained an conditional GAN for this task.

% \begin{equation}
% L_{G} = E_{m_{sim} \sim G_{\theta_M}(z_i), s_{real} \sim P_{data}}[log(1-D(G(s_{real},m_{sim}), c=(s_{real},m_{sim})))]
% \end{equation}

% \begin{equation}
% \begin{split}
% L_{D} = E_{(s_{real}, I) \sim P_{data}, m_{sim} \sim G_{\theta_M}(z_i)}[log(D(I, c=(s_{real},m_{sim})))] + \\
% E_{(s_{real}, I) \sim P_{data}, m_{sim} \sim G_{\theta_M}(z_i)}[1- log(D(G(s_{real},m_{sim}, c=(s_{real},m_{sim})))]
% \end{split}
% \end{equation}

% \subsection{Stage III: Jointly training with label and unlabel data}
% The training of the first two stages only use label data which is expensive to get especially in medical imaging domain. We want to improve our generative model ability by jointly training with label and unlabel data. In Stage I, we have per sample latent representation $zi_{label} \in Z_{label}$ for each image with label. In this stage, we can sample $N_{unlabel}$ $zi_{unlabel} \in Z_{unlabel}$ as initialization latent representation for unlabel data with the intuition that unlabel data and label data come from the same data distribution, thus their latent representation should not be far away from each other. We then jointly train Stage I \& II model with label and unlabel data alternatively. When training with label data, we use a smaller learning rate for all the model parameters as it is already trained before and the purpose of this training is to finetune the parameters and reinforce the learning of the label data. When training with unlabel data, since the Stage I \& II models never see those data before, we use a larger learning rate to encourage the learning process. After jointly training, the shape material model and the conditional generator learn the distribution of unlabel dataset while do not forget what have learnt from label data.
